Embracing Annotation Efficient Learning (AEL) for Digital Pathology and Natural Images

Jitendra Malik once said, "Supervision is the opium of the AI researcher". Most deep learning techniques heavily rely on extreme amounts of human labels to work effectively. In today's world, the rate of data creation greatly surpasses the rate of data annotation. Full reliance on human annotations is just a temporary means to solve current closed problems in AI. In reality, only a tiny fraction of data is annotated. Annotation Efficient Learning (AEL) is a study of algorithms to train models effectively with fewer annotations. To thrive in AEL environments, we need deep learning techniques that rely less on manual annotations (e.g., image, bounding-box, and per-pixel labels), but learn useful information from unlabeled data. In this thesis, we explore five different techniques for handling AEL.

==> 021_deeplearning.tex <==
\section{Deep Learning}\label{sec:dl}

Deep learning can be traced back to the 1960s, when Frank Rosenblatt introduced a feed-forward perceptron, a biologically inspired machine learning model that can solve binary classification problems~\cite{rosenblatt1958perceptron}. Despite its popularity,  there are a few major drawbacks. Firstly, a single  Roseblatt's perceptron cannot solve the eXclusive-OR (XOR) problem, which is linearly non-separable~\cite{block1970review}~\footnote{XOR problem can be solved by having more than one layer~\cite{goodfellow2016deep}.}. Secondly, this simple perceptron requires heuristic weight adjustments that have to be performed for every new task because the optimal weight may differ depending on the tasks.  In 1986, Rumelhart, Hinton, and  Williams~\cite{rumelhart1986learning} popularized backward propagation in a multi-layered perceptron where the weights of a neuron can be tuned automatically with respect to its loss function.   
Later in 1989, Cybenko et al.~\cite{cybenko1989approximation} showed that a feed-forward neural network coupled with a non-linear activation function (Sigmoid) is a universal approximator if it has enough hidden units.  
In 1980, inspired by Hubel and Wiesel's work~\cite{hubel1959receptive} on the receptive field of a single neuron in the visual cortex, Fukushima~\cite{fukushima1980neocognitron} introduced the very first Convolutional Neural Network (CNN), consisting of convolution and downsampling layers. Later in 1989, Le Cun et al.~\cite{lecun1989backpropagation} used backpropagation to update the weights in the convolutional neural networks directly from images of handwritten numbers, showing that automatic weight updates are better than manually hand-crafted convolutional layers.
Despite some success in the 1980s, deep learning research was thwarted by the lack of computation power and data quantity. Deep Learning was superseded by other competitive learning algorithms, such as Support Vector Machines (SVM) and its extensions.

In the late 2000s, deep learning became the dominant algorithm in solving image classification, object detection, and semantic segmentation. In 2009, Deng et al. created a large-scale supervised dataset known as ImageNet~\cite{imagenet_cvpr09}, where they aimed to use big data to promote data-driven pattern recognition. Around the same time, several research groups had started to use Graphics Processor Units (GPU) to accelerate the speed of deep network training~\cite{raina2009large}.
In 2012, deep learning outperformed other learning algorithms by a large margin in the image recognition task where it utilized both a large-scale dataset (ImageNet) and GPU's fast computation speed.
 From 2012 onwards, there has been an extraordinary rise in research on deep learning in the computer vision community.

Most deep learning models are trained in a fully supervised environment, where large amounts of human-annotated data are required~\cite{goodfellow2016deep}. 
Data annotation cost can be astronomical depending on the quantity of unlabeled and the expertise of human annotators. 
It is costly to label all possible data as hundreds of millions of unlabeled data are created daily~\cite{kaiser2020social,amt}.  
Furthermore, domain experts are needed to annotate the data in some domains, such as the medical image domain. The high salary of domain experts further amplifies the data annotation cost~\cite{md_salary}. 
To overcome the need to collect more labeled data, we need a model that can handle an environment where human-annotated data are scarce and limited. Strategies to train deep models in SCADE are reviewed in the following few chapters.


==> 022_data_augmentation.tex <==
\section{Data Augmentation}

%A Deep model can approximate any continuous function given enough capacities. 
A neural network is a universal approximator that can approximate any continuous function if it has enough hidden units~\cite{cybenko1989approximation}. Since a deep model consists of many neural networks, it can easily overfit a given dataset, which is why deep learning requires significant amount of annotated data to be effective.
In a SCarcely Annotated Data Environment (SCADE), where annotated data are limited, data augmentation is an excellent strategy to combat overfitting without collecting more annotations.    
Overfitting can be reduced via simple data augmentation strategies such as random cropping, random rescaling, and image jittering~\cite{krizhevsky2012imagenet}. 
Srivastava et al.~\cite{srivastava2014dropout} discovered Dropout where they randomly zero-outed the signals within a deep network. 
DeVries et al. proposed CutOut, which randomly blocks out a continuous chunk of an image,  providing image-level augmentation during training~\cite{devries2017improved}. Ghiasi et al. proposed Dropblock that randomly blocks out a continuous chunk of feature space, yielding feature-level augmentation during training~\cite{ghiasi2018dropblock}. Zhang et al. proposed MixUp to interpolate between two images and their corresponding annotations~\cite{zhang2018mixup}. Yun et al. proposed CutMix that creates a composite image by combining two images and their corresponding annotations~\cite{yun2019cutmix}. All these augmentation techniques regularize deep learning networks to reduce overfitting and improve generalization~\footnote{The goal of machine learning is to train a model that can perform well to unseen data, a.k.a generalization~\cite{goodfellow2016deep}. Overfitting happens when a model memorizes the training data, and underfitting happens when a model fails to learn from the training data. There is usually a range of sweet spots between overfitting and underfitting, where a decrease in overfitting will yield better generalization. This trade-off is also known as the bias-variance trade-off.}.  

%It is a blessing because we can use a neural network to approximate anything\footnote{see Sec.~\ref{sec:dl} for Universal Approximator's definition.}, but it is a curse as it will easily overfit a given dataset. The main reason why deep learning requires tremendous annotated data to be successful is due to the overfitting problem. 
%Additionally, these augmentation techniques are also used in semi-superivsed learning (Sec.~\ref{sec:semi}) and unsupervised learning (Sec.~\ref{sec:self}). 

%A simple trick, namely Dropout, can regularize a deep network to prevent overfitting~\cite{srivastava2014dropout}. Dropout works by randomly zero-out the signals within a deep network. 

%Srivastava et al.~\cite{srivastava2014dropout} discovered a simple trick, namely Dropout, to regularize a deep network to prevent overfitting, where they randomly zero-outed the signals within a deep network. Coupling with Dropout and simple data augmentation strategies (i.e., random cropping and image jittering), Krizhevsky et al.~\cite{krizhevsky2012imagenet} outperformed other machine learning techniques by a huge margin in the ImageNet competition. DeVries et al.~\cite{devries2017improved}  proposed CutOut, which randomly blocks out a continuous chunk of an image to prevent overfitting. Ghiasi et al.~\cite{ghiasi2018dropblock} proposed Dropblock, which randomly blocks out a continuous chunk of feature space. Zhang et al.~\cite{zhang2018mixup} proposed Mixup to interpolate between two images and their corresponding annotations. Yun et al.~\cite{yun2019cutmix} proposed CutMix, which creates a composite image by combining two images and its corresponding annotations. All these augmentation techniques not only improve supervised learning, they are also used in semi-superivsed learning (Sec.~\ref{sec:semi}) and unsupervised learning (Sec.~\ref{sec:self}). 

==> 023_metric_learning.tex <==
\section{Metric Learning}\label{sec:metric}

%Searching is the fundamental of knowledge. In order to search for something in a given dataset, we need to have a good metric to compare and contrast each sample in the dataset. 

%Distance metric learning (DML), aims to improve the generalization of representation of pre-trained models (models trained on a source dataset) that goes beyond classic cross-entropy loss. 
%The core idea of DML is to learn an embedding space where similar examples are attracted and dissimilar examples are repelled. 
%In this subsection, we limit our review to methods that consider image retrieval. 
%There is a large body of work in DML, and it can be traced back to the 90s, where Bromley et al.~\cite{Bromley:1993:SVU:2987189.2987282} designed a Siamese neural network to verify signatures.
%where pairs of similar and dissimilar images are selected, and the distance between similar pairs of images is minimized while the distance between dissimilar images is maximized.
%Like contrastive loss, which deals with the actual distance between two images, 
%where pairs of similar and dissimilar images are selected, and the distance between similar pairs of images is minimized while the distance between dissimilar images is maximized.
%Like contrastive loss, which deals with the actual distance between two images, 
%In addition to contrastive and triplet loss, there is a long line of work which proposes new loss functions, such as angular loss~\cite{Wang_2017_ICCV}, histogram loss~\cite{NIPS2016_6464}, margin-based loss~\cite{wu2017sampling}, and hierarchical triplet loss~\cite{Ge_2018_ECCV}. Wang et al.~\cite{wang2019multi}~categorize this group as paired-based DML.
%Song et al. proposed lifted embedding training to utilize all pair-wise samples in a mini-batch to form triplets, where each positive pair compares its distance with all negative pairs~\cite{song2016deep}. Models trained with lifted embedding training outperform models trained with contrastive and triplet loss. 

Distance metric learning (DML) is a type of learning that learns an embedding space where similar examples are attracted and dissimilar examples are repelled. DML can be executed in a supervised or unsupervised fashion. Supervised DML can improve the generalization of features and is often applied to image retrieval, facial recognition, and object re-identification tasks~\cite{wang2019multi,Schroff_2015_CVPR,song2016deep,liu2016deepfashion}. 
%Unsupervised DML in the form of consistency loss and contrastive loss are commonly used techniques in semi-supervised and unsupervised learning (Chapter~\ref{sec:semi} and~\ref{sec:self})


\subsection{Zero-shot image retrieval with Distance Metric Learning}~\label{sub:rel_dml}

\noindent Zero-shot image retrieval is a task where images of unseen classes are retrieved. During training, a model is trained with a set of images with known classes, and the goal is to cluster images of unknown classes.
Zero-shot image retrieval is an important problem because it examines the generalizability of a model on unknown classes. Distance metric learning (DML) is commonly used to solve zero-shot image retrieval task. 
Where labeled data is scarce, DML improves the generalization of a model without additional labeled data~\cite{liu2019large}. 


DML can be tackled via pair-based methods, where we compare images directly with one another~\cite{wang2019multi}. Contrastive loss minimizes the absolute distance between a pair of similar images and maximizes the absolute distance between a pair of dissimilar images~\cite{chopra2005learning,hadsell2006dimensionality}. Triplet loss offers a richer comparison between images by optimizing the relative distance between a positive pair~\footnote{An anchor image and an image similar to anchor image.} and a negative pair~\footnote{An anchor image and an image dissimilar to anchor image.} of images~\cite{Chechik:2010:LSO:1756006.1756042}. 
Multi-class N-pair loss improves the cohesiveness of similar images by repelling an anchor~\footnote{An anchor image is defined as an image selected during training that acts as a reference point to other images.} image against multiple dissimilar images~\cite{sohn2016improved}. 
Lifted embedding loss increases the number of comparisons between images in a single batch by utilizing all pair-wise samples in a mini-batch to form triplets, where each positive pair compares its distance with all negative pairs~\cite{song2016deep}. All these pair-based methods show that DML can be improved via a richer comparison between images.  

%In the 90s, DML was used to verify signatures via a siamese network~\cite{Bromley:1993:SVU:2987189.2987282}. 
%Later, DML was used in facial recognition, and dimensionality reduction in the form of a contrastive loss, where the actual distance between two images are optimized~\cite{chopra2005learning,hadsell2006dimensionality}. Triplet Loss was proposed to optimize the relative distance between a positive pair~\footnote{An anchor image and an image similar to anchor image.} and a negative pair~\footnote{An anchor image and an image dissimilar to anchor image. An achor image is defined as an image selected during training that acts as a reference point to other images.} of images~\cite{Chechik:2010:LSO:1756006.1756042}. 
%In addition to contrastive and triplet losses, a series of works proposed new loss functions to improve the comparison of images, such as angular loss~\cite{Wang_2017_ICCV}, histogram loss~\cite{NIPS2016_6464}, margin-based loss~\cite{wu2017sampling}, and hierarchical triplet loss~\cite{Ge_2018_ECCV}. Wang et al.~\cite{wang2019multi}~categorized this group as paired-based DML, which compares images directly with one another. 

Several works had been proposed to explore more efficient data sampling strategies for pair-based methods. Schroff et al. explored a curriculum learning strategy where examples are selected based on the distances of samples to the anchored images~\cite{Schroff_2015_CVPR}. They used a semi-hard negative mining strategy to select negative samples where the distances between negative pairs are at least greater than the positive pairs. However, such a method usually generates very few semi-hard negative samples, and thus requires very large batches (on the order of thousands of samples) in order to be effective.
Wu et al. proposed a distance-based sampling strategy where examples are sampled based on inverse $n$-dimensional unit sphere distances from anchored samples~\cite{wu2017sampling}. This sampling strategy addresses the issue of uniform random sampling, which yields highly redundant samples.
Wang et al. proposed a mining and weighting scheme, namely multi-similarity scheme (MS), where informative pairs are sampled by measuring positive relative similarity, and then further weighted using self-similarity and negative relative similarity~\cite{wang2019multi}. Models trained with samples picked by MS yield better image retrieval performance when compared to models trained with other sampling strategies such as random sampling~\cite{oh2016deep}, curriculum-based sampling~\cite{Schroff_2015_CVPR} and distance-based sampling~\cite{wu2017sampling}. 
%These works~\cite{Schroff_2015_CVPR,wu2017sampling,wang2019multi} showed that 
In short, data sampling is a crucial component in pair-based DML and can improve performance significantly. 

%Apart from pair-based DML methods, there were other works that tackled DML via proxies, which were used to estimate class distribution. 
DML can also be tackled by comparing samples with proxies. Proxies are used to represent samples of similar classes.  Proxies allows a richer comparison of images by comparing an image to an image distribution (e.g., class mean) instead of comparing images with one another. As a result, proxies can also reduce computation costs. Cluster centroids serve as proxies in magnet loss where samples are attracted to cluster centroids of similar classes and repelled by cluster centroids of different classes~\cite{rippel2015metric}. In ProxyNCA, learnable proxies in the form of updatable parameters are used to represent class distribution~\cite{movshovitz2017no}. During training, each sample is pushed towards its proxy while repelling  all other proxies of different classes.
Similar to ProxyNCA, Zhai et al.~\cite{zhai2019} designed a proxy-based solution using Cosine distance rather than the Euclidean squared distance. They used layer norm in their model to improve robustness against poor weight initialization of new parameters and introduced class balanced sampling during training that improves the image retrieval performance of Proxy-based DML solutions. 
In brief, DML's performance can be improved by utilizing class distribution in image comparison. 
%There are significantly fewer works that explored proxy-based DML when compared to paired-based DML. 
%In Sec.~\ref{sec:eccv} we revisit proxy-based DML methods and propose a few enhancements. 

% ProxyNCA. 
%Magnet loss was proposed to minimize the distance between samples and cluster centroids of similar classes and maximize the distance between samples and cluster centroids of different classes~\cite{rippel2015metric}. 


%Apart from methods dedicated to addressing the weakness of pair-based DML methods, 
%Apart from pair-based DML methods, there were other works that tackled DML via class distribution estimation. 
%There were another line of works that tackled DML via class distribution estimation. 
%The motivation is to compare samples to proxies, and in doing so, reduce computation cost. 
%One method that falls under this line of work is the Magnet Loss~\cite{rippel2015metric}, in which samples are associated with a cluster centroid, and at each training batch, samples are attracted to cluster centroids of similar classes and repelled by cluster centroids of different classes. Another method in this camp is ProxyNCA~\cite{movshovitz2017no}, where proxies are stored in memory as learnable parameters. During training, each sample is pushed towards its proxy while repelling against all other proxies of different classes. %ProxyNCA is discussed in greater detail in Section \ref{sec:proxynca}.
%Similar to ProxyNCA, Zhai et al.~\cite{zhai2019} designed a proxy-based solution that used Cosine distance rather than the Euclidean squared distance. They also used layer norm in their model to improve robustness against poor weight initialization of new parameters and introduced class balanced sampling during training, which improves their retrieval performance. 
%In Sec.~\ref{sec:eccv} we revisit ProxyNCA and propose six enhancements to improve ProxyNCA. 

%Recently, a few works in DML have explored ensemble techniques. Opitz et al.~\cite{Opitz_2017_ICCV} train an ensemble by reweighting examples using online gradient boosting. The downside of this technique is that it is a sequential process. Xuan et al.~\cite{xuan2018deep} address this issue by proposing an ensemble technique where ensemble models are trained separately on randomly combined classes. Sanakoyeu et al.~\cite{sanakoyeu2019divide} propose a unique divide-and-conquer strategy where the data is divided periodically via clustering based on current combined embedding during training. Each cluster is assigned to a consecutive chunk of the embedding, called learners, and they are randomly updated during training. Apart from ensemble techniques, there is recent work that attempts to improve DML in general. Jacob et al.~\cite{jacob2019metric} discover that DML approaches that rely on Global Average Pooling (GAP) potentially suffer from the scattering problem, where features learned with GAP are sensitive to outliers. To tackle this problem, they propose a high-order regularizer for deep embeddings (HORDE) that computes higher-order moments of features.



==> 023_transfer_learning.tex <==
\section{Transfer Learning}~\label{sec:tl}

%Transfer learning is a type of machine learning strategy where we aim to learn a meaningful representation from a source dataset so that these representations can be transferred to a target dataset. 
Transfer Learning is a type of machine learning strategy where knowledge is transferred from a source dataset to a target dataset. 
With the help of a large scale supervised dataset like ImageNet~\cite{imagenet_cvpr09}, deep learning can extend its reach through transfer learning to solve many computer vision problems such as object detection, object segmentation, object tracking, image retrieval, and many more.
 In deep learning, fine-tuning is the most common form of transfer learning due to ImageNet pre-trained models' effectiveness in capturing high-level features. 
 To be specific, we refer to fine-tuning (heterogeneous transfer learning), where the source and target dataset have different tasks, and the features are transferred via the weights of a model trained on the source dataset.
 Other forms of transfer learning are outside the scope of this work, such as domain adaption~\cite{wang2018deep}. 
 Without transfer learning, more labelled images are needed during training. Therefore, transfer learning via fine-tuning is a good strategy, where labeled data is sparse and limited~\cite{huh2016makes}. 
 %Section~\ref{sec:isbi} shows an example where a model can performed better than a randomly initialized model via transfer learning in SPADE. 

%There are many forms of transfer learning but we are limiting our scope to the most common form of transfer learning which is known as heterogeneous transfer learning.  
%~\cite{girshick2014rich}
%~\cite{chen2017deeplab}
%~\cite{teh2020proxynca++}

==> 024_semisupervised_learning.tex <==
\section{Semi-supervised Learning}\label{sec:semi}

Semi-supervised learning is a fundamental topic in machine learning. It allows models to learn useful representations with a few human labels, abling them to reduce the reliance on manual data annotation. 
This property is advantageous when labeled data is limited but unlabeled data is abundant.  
%While this topic is far from solved, much progress in semi-supervised classification had been witnessed in the past few years. 
One common way of handling semi-supervised learning is to minimize consistency loss between two outputs of the same image via various augmentations. For instance, training a model with consistency loss via input and feature perturbations was shown to be an effective strategy for semi-supervised classification~\cite{sajjadi2016regularization}. Additionally, temporal ensembling provided a new dimension for feature comparison yielding a performance gain when coupled with input and feature perturbations~\cite{laine2016temporal}. With temporal ensembling, a model compares its features computed in the current iteration with their corresponding temporal ensembled features, which are the exponential moving averages of features computed from previous iterations. 
A mean teacher model was further proposed by computing the model's weights via an exponential moving average of the model's weight from previous iterations \cite{li2020unsupervised}. Consistency loss via a mean teacher model yielded a higher performance compared to the temporal ensembling method. 
%These works~\cite{sajjadi2016regularization,laine2016temporal,tarvainen2017mean} show that 
In short, there are various ways to compute consistency loss for semi-supervised classification. 

Another way of tackling semi-supervised learning is via data interpolation. 
MixUp was proposed to interpolate between two labeled images via linear combinations of both the input and label space~\cite{zhang2018mixup}. The distribution of the composite images and labels follows a beta distribution which is heavily weighted towards one or the other images and their corresponding labels. MixMatch further extends MixUp to unlabeled images by interpolating between labeled images and unlabeled images~\cite{berthelot2019mixmatch}. In MixMatch, label sharpening was proposed to improve the predictions of unlabeled images by taking the average predictions of perturbed unlabeled images. 
Additionally, ReMixMatch was proposed to further improve the predictions of unlabeled images by aligning the marginal distribution of unlabeled images and labeled images \cite{li2020unsupervised}. 
%These works~\cite{zhang2018mixup,berthelot2019mixmatch,berthelot2019remixmatch} show that 
In summary, a better prediction of unlabeled data will yield a more accurate data interpolation between labeled and unlabeled data resulting a boost in performance for semi-supervised classification. 

Recently, there has been a resurgence of using self-training for semi-supervised learning. 
Self-training or pseudo-labeling is a classic semi-supervised learning method that uses pseudo-labels to guide the process of learning. Pseudo-labels are defined as labels computed by a model. A major benefit of self-training is that it allows easy extension from an existing supervised model without discarding any information. In 1996, self-training was used to solve semi-supervised sentence classification by iteratively adding unlabeled data to labeled data via pseudo-labeling~\cite{yarowsky1995unsupervised}. 
The introduction of joint loss between labeled and unlabeled data via pseudo-labels popularized self-training in the deep learning literature~\cite{lee2013pseudo}. During training, pseudo-labels were gradually integrated into the joint loss by increasing the weight of unlabeled data via an iteration-dependent co-efficient.  After the re-appearance of self-training, it has gained traction in recent years. Mixture of all models (MOAM) was shown to be an effective way to tackle semi-supervised classification via the integration of unsupervised learning and self-training training~\cite{zhai2019s4l}. 
Additionally, self-training was shown to improve a randomly initialized model outperforming a pre-trained model on object detection~\cite{zoph2020rethinking}. 
Self-training with noisy pseudo-labels via random augmentations improves a classification model's accuracy and robustness~\cite{xie2020self}. Self-training via pseudo-labels ensembling also surpasses a supervised model in a omni-supervised learning environment that includes out-of-distribution samples during training~\cite{radosavovic2018data}.  
%All these recent works show that 
In brief, self-training is a competitive alternative to tackle semi-supervised learning. 


\subsection{Semi-supervised Semantic Segmentation}~\label{sec:semi_seg}

%From Sec.~\ref{sec:semi}, we witness a plethora of work for semi-superivsed classification, however, many of these solutions rely on augmentation strategies that alter spatial information, which may harm semantic segmentation tasks. In this subsection, we look into semi-supervised techniques for semantic segmentation. 
Semi-supervised semantic segmentation is the task of producing pixel-wise semantic labels given only a small number of human annotated training examples. 
%This task aligns with SPADE, where human annotation is limited. 
%Semi-supervised semantic segmentation has gained ground in recent years. 
Souly et al.~\cite{souly2017semi} extended a typical Generative Adversarial Network (GAN) network by designing a discriminator that accepts images as input and produces pixel-wise predictions consisting of confidence maps for each class and a fake label. Hung et al.~\cite{hung2019adversarial} improved GAN-based semantic segmentation by using a segmentation network as a conditional generator.  They also redesigned the discriminator to accept the segmentation mask as input and restricted it to produce pixel-wise binary predictions. Mittal et al.~\cite{mittal2019semi} extended Hung et al.'s network by making the discriminator produce an image-level binary prediction, adding a feature matching loss and self-training loss in their training pipeline. The most notable addition was the proposal of a separate semi-supervised classification network~\cite{tarvainen2017mean} to clean up the prediction of segmentation masks. 
%These works~\cite{souly2017semi,hung2019adversarial,mittal2019semi} show that 
In short, GAN can be adapted to handle semi-supervised semantic segmentation. 

A few works proposed non-GAN based solutions for semi-supervised semantic segmentation. Mendel et al.~\cite{mendelsemi} proposed an error-correcting network that aimed to fix the predictions of the main segmentation network. This error-correcting network was also applied to unlabeled images to correct the generated mask.
French et al.~\cite{french2019semi} adapted CutMix~\cite{yun2019cutmix} to augment and regularize a segmentation network by creating composite images via mixing two different images and their corresponding segmentation masks.
Similarly, Olsson et al.~\cite{olsson2020classmix} regularized the segmentation network by mixing segmentation masks from two images by selecting half of the classes from one image and the other half from another image.
Ouali et al.~\cite{Ouali_2020_CVPR} minimized consistency loss between features of multiple auxiliary decoders in which the perturbed encoder outputs were fed. In summary, semi-supervised semantic segmentation can be tackled 
with non-GAN based techniques that often borrow the same ideas from semi-supervised classification. 
%by revisiting semi-supervised methods for classification, such as consistency loss and data augmentation. 

%non-GAN based techniques~\cite{mendelsemi,french2019semi,olsson2020classmix,Ouali_2020_CVPR} are useful in handling semi-supervised semantic segmentation. 
%In Sec.~\ref{sec:iccv} we explore iterative self-training for semi-supervised semantic segmentation. 

% In Section~\ref{sec:cvpr}, we also explore a non-GAN based solution, namely self-training, to tackle semi-supervised semantic segmentation. Self-training or pseudo-labeling is a classic semi-supervised learning recipe that can be traced back to 1996, where it was used in an NLP application~\cite{yarowsky1995unsupervised}. A major benefit of self-training is that it allows easy extension from an existing supervised model without discarding any information.
% In the deep learning literature, Lee et al.~\cite{lee2013pseudo} popularized self-training in semi-supervised classification. After its re-appearance, it has gained traction in recent years. Zhai et al.~\cite{zhai2019s4l} show the effectiveness of mixing self-supervised and semi-supervised learning along with pseudo-labeling in their training regime. Zoph et al.~\cite{zoph2020rethinking} show that a randomly initialized model with self-training via a joint-loss can yield better performance than a model initialized with a pre-trained model without self-training. Xie et al.~\cite{xie2020self} show that iterative self-training with noisy labels improves a classification model's accuracy and robustness.
% Radosavovic et al.~\cite{radosavovic2018data} use self-training in Omni-supervised learning where they generate pseudo-labels by taking the average prediction of multiple perturbations of a single unlabeled image.

% Most of the recent self-training works~\cite{lee2013pseudo,radosavovic2018data,zhai2019s4l,zoph2020rethinking} are confined to only one refinement stage, with the exception of Xie et al.'s work~\cite{xie2020self}, where they benefit from iterative self-training by repeating self-training for three stages of refinement.
% In our work (see section~\ref{sec:cvpr}), we aim to extend self-training for semi-supervised semantic segmentation and investigate self-training behavior under many (i.e.~$>3$) refinement stages.\looseness=-1

==> 025_selfsupervised.tex <==
\clearpage
\section{Unsupervised Learning}~\label{sec:self}

Unsupervised learning is the holy grail of deep learning. The aim of unsupervised learning is to learn representations without any human labels. This goal aligns with the theme of handling SPADE, where labeled data is scarce and unlabeled data is abundant. 
A new buzzword for unsupervised learning that emerged recently is self-supervised learning. Self-supervised learning can be viewed as a subset of unsupervised learning that relies on itself (input) as a supervision~\cite{grill2020bootstrap}. In this thesis proposal, unsupervised learning includes both unsupervised and self-supervised learning. 
%The following are non-exhaustive reviews of unsupervised learning work grouped by methods.  
One way to perform unsupervised learning is via input reconstructions. 
Hinton et al. created an autoencoder where a neural network learns to encode an input image to a lower dimension and then reconstruct the input image by decoding the lower dimension code~\cite{hinton2006reducing}. Vincent et al. proposed a denoising autoencoder, where a neural network learns to reconstruct an image from a noisy image~\cite{vincent2008extracting}. Mikolov et al. designed WordVector, where a neural network learns to predict a word given surrounding words~\cite{mikolov2013distributed}. Similarly. Pathak et al. created a context autoencoder where a deep network learns to reconstruct an image patch given the surrounding image patches~\cite{pathak2016context}. 
%These works show that 
In brief, meaningful features can be learned via input reconstructions without any human supervision. 

Another way to perform unsupervised learning is by learning the position of image patches. 
Doersch et al. proposed to learn the relative position of two image patches. Given a center image patch and a random image patch, the model has to predict the direction of the random image path with respect to the center image patch~\cite{doersch2015unsupervised}. 
Noroozi et al. learned representation by predicting the identity of jigsaw puzzles~\cite{noroozi2016unsupervised}. They generated K permutations of puzzles for each image and then trained a model to predict the puzzle id for each unique permutation. 
Gidaris et al. performed representation learning by predicting the rotation angle of a randomly rotated image~\cite{gidaris2018unsupervised}. During training, they randomly rotated the input images and asked the model to predict the rotation angles. In summary, meaningful features can be learned by learning the position of image patches without any human supervision. 

Unsupervised metric learning with contrastive loss and consistency loss is another group of methods to perform unsupervised learning. 
Chen et al. designed a contrastive learning method, SimCLR, to minimize the distance between an image and its perturbed copy and maximized the distance between a given image and a subset of other images in the dataset~\cite{chen2020simclr}. 
Grill et al. used a consistency loss similar to Mean Teacher~\cite{tarvainen2017mean} where they minimized the features between a student and a teacher model~\cite{grill2020bootstrap}. In a nutshell, useful features can be learned via contrastive and consistency loss that do not require human annotations. 

Clustering does not require human supervision and can also be used as supervision in unsupervised learning. %Additionally, some works focused on using clustering as supervision in unsupervised learning. 
Xie et al. designed deep embedded clustering (DEC) where a deep network learns to learn representation and perform clustering simultaneously~\cite{xie2016unsupervised}. Guo et al. further improved DEC by incorporating a denoising autoencoder to DEC~\cite{guo2017improved}. Caron et al. created DeepCluster, where they use a deep network to predict pseudo-labels generated via clustering~\cite{caron2018deep}. They repeated this process multiple times by performing clustering and classification in the new feature space resulting in a competitive solution despite its simplicity. Yan et al. proposed ClusterFit, where they performed clustering using pre-trained features and then trained a deep network using pseudo-labels generated via clustering~\cite{yan2020clusterfit}. Yan et al. showed that ClusterFit could learn better transferable features than networks that rely only on human-annotated labels. 
%These works~\cite{xie2016unsupervised, guo2017improved,caron2018deep,yan2020clusterfit} exploit clustering and show that meaningful features can be learned without human supervision. 
In summary, clustering is useful for learning meaningful features without human supervision. 

%\newpage



==> 026_histology.tex <==
\section{Digital Pathology}~\label{sec:dp}

Digital Pathology (DP) is a field of medical imaging where microscopic images are analyzed. 
%The introduction of hardware for a complete digital telepathology system allowed whole slide images (WSI) to be widely available~\cite{pantanowitz2010digital}.  
Most machine learning and computer vision works are designed to handle Natural Image (NI) tasks. However, there are distinctions between NI and DP domains. 
One key difference between DP and NI domain is the image size. In DP, each WSIs are usually giga-pixels in size, whereas in NI, each image is usually mega-pixels in size. Another key difference is that a coarse-grain view (seeing the whole image) conveys little to no meaningful information in DP. In NI, a human can describe the content of an image just by viewing the whole image.
%Hence, methods of training model without additional human annotation 
Additionally,  NI images as a whole are often use directly for machine learning training. In DP, researchers usually divide each giga-pixel image into small patches at various zoom-level~\cite{45922,aresta2019bach}. After converting WSI to image patches, a standard pipeline in deep learning can be used for training. 
In NI, human annotations are relatively inexpensive when compared to DP because the annotation can be completed by laypersons. 
In DP, the cost of human annotation increases by a large margin because annotations are obtained from medical experts that required specialized knowledge~\cite{md_salary,45922}. 
The high annotation cost of DP highlights the importance of handling SPADE, where human annotations are limited. 

%Semi-supervised and unsupervised learning are important methods to handle SPADE.Li et al.~\cite{li2018based} explored Expectation Maximization (EM) based approach for semi-supervised semantic segmentation in DP where they trained a deep segmentation model using labels generated by the expectation step of the EM algorithm. Their EM-based semi-supervised approach yielded a higher performance in cancer segmentation when compared to the supervised baseline. 
%Srinidhi et al.~\cite{srinidhi2021selfsupervised} proposed a Resolution Sequence Prediction (RSP) task for unsupervised learning in DP, where they trained a model to predict the sequence of patches with various magnification levels. RSP outperformed other unsupervised learning methods such as MoCo~\cite{he2020momentum} and VAE~\cite{kingma2013auto} in breast cancer classification.  Ciga et al.~\cite{ciga2020self} showed that using WSI from multiple organs helps to improve the performance of unsupervised learning. Jaiswal et al.~\cite{jaiswal2019semi} showed that self-training with WSI extracted unlabelled images can improve supervised breast cancer classification performance. Lu et al.~\cite{lu2019semi} performed semi-supervised learning for breast cancer classification by combining contrastive loss (CL) and multiple instance learning (MIL), where they used an attention mechanism to attend to the cancer positive image patches. The combination of MIL and CL yields a significant boost in performance compared to MIL alone. In short, useful features can be learned without additional human supervision in DP.    
\clearpage


==> 03_midl.tex <==
\section{Metric Learning for Patch Classification in Digital Pathology}\label{sec:midl}
In digital pathology (DP), classifying gigapixel-sized whole slide images (WSI) is a very challenging task. Many off-the-shelf methods will not work directly with DP because resizing gigapixel images loses granular information, which is vital in differentiating between normal and tumor cells. Moreover, processing entire gigapixel images directly poses algorithmic and computational challenges. A commonly used pipeline first identifies tissue regions in WSI. This is followed by extracting patches that correspond to tissue and training a patch tumor classifier, which is then used to generate a heatmap for the WSI. Finally, another tumor classifier is trained using the morphological and geometrical information from the thresholded heatmap as features to classify WSI.

Current techniques \cite{liu2017detecting, lee2018robust, wang2016deep} for patch classification in DP optimize the cross-entropy loss. However, these techniques do not exploit comparison between data samples which we hypothesize is a useful way to regularize the network.

Metric Learning is a task to learn the similarity and dissimilarity between examples. It is commonly used for re-identifying objects such as people~\cite{rahman2017person}, animals~\cite{deb2018face} or insects~\cite{murali2019classification}. In the context of classification, the benefit of metric learning over traditional setups (e.g.~softmax) is that it does not assume the number of individuals to be fixed. Recently, metric learning has also been used in semi-supervised learning~\cite{laine2016temporal, tarvainen2017mean}, which allows a model to be trained with little supervised information by utilizing unlabeled data. Conventionally, features are learned by training an auto-encoder on the unlabeled data where the difference between original image and reconstructed image is minimized \cite{rasmus2014denoising}. With metric learning, features can be learned by self-comparison under different perturbations.

\bigskip

\noindent{\textbf{Contribution:}} We use metric learning to improve the generalization of patch tumor classification models. Specifically, we learn two distance metrics: a) distance between perturbed samples and b) distance between samples from the same classes and different classes. We show that both distance metrics can be optimized together yielding a stacking improvement over one another.

Our proposed models are illustrated in Fig.~\ref{fig:model}.

\begin{figure}[ht]%htb
\centering
{\setlength{\tabcolsep}{2pt}
\scalebox{0.75}{
\includegraphics[width=4.2in]{figs/pi_net.pdf}
}
}
\caption{The proposed models: {\color{green}{Pi}} and {\color{orange}{Pi+}}. The Pi model uses the self-perturbation loss which is the mean squared distance between the classification outputs of perturbed samples. The Pi+ model uses an additional loss function, contrastive loss which minimizes intra-class differences and maximizes inter-class differences.}
\label{fig:model}
\end{figure}

\subsection{Methods}
Our method uses a standard CNN-based softmax classifier augmented with additional losses.

\bigskip

%Laine et al. coined their framework as the Pi model.
\noindent{\textbf{Self-Perturbation Loss:}} One way to learn the similarity between samples is by self-comparison. This can be achieved by minimizing the differences between the same sample under different perturbations \cite{laine2016temporal}.  Let $x_i$ be a training example and $z_i$ and $z_i^*$ be the pre-softmax predictions of $x_i$ under different perturbations. Perturbation in our experiment is done via data augmentation which is described in Sec.~\ref{sec:exp}.
Self-Perturbation Loss, $L_1$ is defined as the mean squared differences between $z_i$ and $z_i^*$.

\begin{equation}\label{eq:11}
 L_1 = \frac{1}{N} \sum_{i}^N (z_i - z_i^*)^2
\end{equation}

\bigskip

\noindent{\textbf{Contrastive Loss:}}
Another way to learn the distance metric between samples is via contrastive learning. Koch et al.~introduced the use of the contrastive loss in a Siamese Network for the one-shot learning task \cite{koch2015siamese}. Let $x_i$ and $x_j$ be two randomly chosen inputs with $y_i$ and $y_j$ labels and $z_i$ and $z_j$ the pre-softmax prediction of $x_i$ and $x_j$. The distance between $z_i$ and $z_j$ is defined as $\text{Dist}(i,j) = \frac{1}{N} \sum_{i}^N (z_i - z_j)^2$. The contrastive Loss, $L_2$ is defined as:

\begin{equation}\label{eq:22}
 L_2 = \frac{1}{N} \sum_{i} \mathbbm{1}{(y_i = y_j)} * \text{Dist}(i,j)) + \mathbbm{1}{(y_i \ne y_j)} * \max(0, 1 - \text{Dist}(i,j))
\end{equation}

\subsection{Experiments}
\noindent{\textbf{Dataset:}}
We experimented on PCam, a subset of the CAMELYON16 dataset~\cite{bejnordi2017diagnostic}, which consists of  CAMELYON16 image patches at 10$\times$ magnification with a train/validate/test split of $74/12.5/12.5\%$. There are $327,680$ total patches of size $96 \times 96$ pixels. Similar to \cite{veeling2018rotation}, we trained our model on the training set and use the validation set for hyper parameter tuning. We reported our results on the test set.

\bigskip

\noindent{\textbf{Experiment Settings:}}\label{sec:exp}
ResNet-34~\cite{He_2016_CVPR} architecture is used in all of the experiments. The models were trained using the Adam optimizer~\cite{kingma2014adam} with an initial learning rate of $1e^{-4}$ for 10 epochs. The learning rate is reduced by a factor of $10$ at the 6th epoch. During training, various data augmentations were performed, these include: a) Random Cropping b) Random Horizontal Flip c) Random Rotation ($0^\circ$ to $360^\circ$) and d) Color Jittering. In detail, we use Pytorch Deep learning framework in our experiments. We also use TorchVision package for data augmentation. Random cropping of size $224 \times 224$ were performed on padded images ($256 \times 256$), where the padded regions are generated via reflection.  Color jittering was performed by setting the brightness, contrast, saturation and hue to 0.4. The best performing model on validation data is kepted at each epoch.
During testing, images were resized to $224 \times 224$ without any augmentation.

\bigskip

\newsavebox\CBox
\def\textBF#1{\sbox\CBox{#1}\resizebox{\wd\CBox}{\ht\CBox}{\textbf{#1}}}

\begin{table}[ht]
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{*8c}
\toprule
Method & Accuracy & Confidence Interval & Significance Test (p-value)\\ \hline
Baseline & 89.21 $\pm$ 0.56 & (88.81, 89.61) & ---\\ \hline
Pi & \textBF{89.94} $\pm$ 0.34 & (89.69, 90.18) & 0.003\\ \hline
Pi+ & \textBF{90.36} $\pm$ 0.41 & (90.06, 90.65) & 0.024\\\hline
P4M\cite{veeling2018rotation} & 89.80 & --- & ---\\
\bottomrule
\end{tabular}
\bigskip

    \caption{Accuracy of our models on PCam dataset. The experiment was run 10 times with different random seeds and we report the mean and standard deviation for each method. We also compared our models with P4M, which is the state-of-the-art architecture. In addition, we also we report 95\% confidence interval for each method and perform significance testing for a) Baseline vs Pi~(row 2) b) Pi vs Pi+~(row 3). The p-values indicate that the results are statistically significant.}
    \label{table:exp_11}

\end{table}

\noindent{\textbf{Results:}}
The results of the experiments are shown in Table~\ref{table:exp_11}, where the mean accuracy and standard deviation were reported. We see that the Pi model outperforms the baseline model. In addition, Pi+ model is better than Pi model and is able to outperform the state-of-the-art architecture~\cite{veeling2018rotation}.

\subsection{Conclusion}
The experimental results showed that both distance metrics can be optimized together yielding a stacking improvement over one another.
This work suggests that metric learning works in DP. Future work could focus on advanced metric learning methods, semi-supervised learning and image retrieval problems.

